Graph-based Features for Automatic Online Abuse Detection

While online communities have become increasingly important over the years, the moderation of user-generated content is still performed mostly manually. Automating this task is an important step in reducing the financial cost associated with moderation, but the majority of automated approaches strictly based on message content are highly vulnerable to intentional obfuscation. In this paper, we discuss methods for extracting conversational networks based on raw multi-participant chat logs, and we study the contribution of graph features to a classification system that aims to determine if a given message is abusive. The conversational graph-based system yields unexpectedly high performance , with results comparable to those previously obtained with a content-based approach.

==> ps-fig.tex <==
% display a postscript figure
\newcommand{\psfig}[5]{
	%
	% \psfig
	% {label}		label for cross referencing
	% {filename.ps}		name of postscript file
	% {caption-adj}		vspace adj (inches) before caption
	% {caption}		text of caption below fig
	% {location}		h (here), t (top of next page),
	%			b (bottom of next page), and/or
	%			p (separate page w/ only figs & tables)
	%
	\begin{figure}[#5]
	\begin{center}
	\leavevmode\epsfbox{#2}
	\vspace{-#3in}
	\caption{#4}
	\end{center}
	\label{#1}
	\end{figure}
}

% display a postscript figure, specifying the width for scaling
\newcommand{\psfigx}[6]{
	%
	% \psfig
	% {label}		label for cross referencing
	% {filename.ps}		name of postscript file
	% {caption-adj}		vspace adj (inches) before caption
	% {caption}		text of caption below fig
	% {location}		h (here), t (top of next page),
	%			b (bottom of next page), and/or
	%			p (separate page w/ only figs & tables)
	% {width}		desired width of fig (inches)
	%
	\begin{figure}[#5]
	\begin{center}
	\epsfxsize = #6 in
	\leavevmode\epsfbox{#2}
	\end{center}
	\vspace{-#3in}
	\caption{#4}
	\label{#1}
	\end{figure}
}

% display a postscript figure, specifying the height for scaling
\newcommand{\psfigy}[6]{
	%
	% \psfig
	% {label}		label for cross referencing
	% {filename.ps}		name of postscript file
	% {caption-adj}		vspace adj (inches) before caption
	% {caption}		text of caption below fig
	% {location}		h (here), t (top of next page),
	%			b (bottom of next page), and/or
	%			p (separate page w/ only figs & tables)
	% {height}		desired height of fig (inches)
	%
	\begin{figure}[#5]
	\begin{center}
	\epsfysize = #6 in
	\leavevmode\epsfbox{#2}
	\vspace{-#3in}
	\caption{#4}
	\end{center}
	\label{#1}
	\end{figure}
}

